Generative artificial intelligence in ophthalmology: multimodal retinal images for the diagnosis of Alzheimer's disease with convolutional neural networks

Background/Aim. This study aims to predict Amyloid Positron Emission Tomography (AmyloidPET) status with multimodal retinal imaging and convolutional neural networks (CNNs) and to improve the performance through pretraining with synthetic data. Methods. Fundus autofluorescence, optical coherence tomography (OCT), and OCT angiography images from 328 eyes of 59 AmyloidPET positive subjects and 108 AmyloidPET negative subjects were used for classification. Denoising Diffusion Probabilistic Models (DDPMs) were trained to generate synthetic images and unimodal CNNs were pretrained on synthetic data and finetuned on real data or trained solely on real data. Multimodal classifiers were developed to combine predictions of the four unimodal CNNs with patient metadata. Class activation maps of the unimodal classifiers provided insight into the network's attention to inputs. Results. DDPMs generated diverse, realistic images without memorization. Pretraining unimodal CNNs with synthetic data improved AUPR at most from 0.350 to 0.579. Integration of metadata in multimodal CNNs improved AUPR from 0.486 to 0.634, which was the best overall best classifier. Class activation maps highlighted relevant retinal regions which correlated with AD. Conclusion. Our method for generating and leveraging synthetic data has the potential to improve AmyloidPET prediction from multimodal retinal imaging. A DDPM can generate realistic and unique multimodal synthetic retinal images. Our best performing unimodal and multimodal classifiers were not pretrained on synthetic data, however pretraining with synthetic data slightly improved classification performance for two out of the four modalities.

==> Figures/DDPM_schema.tex <==
\begin{figure}[H]
\centering
\includegraphics[width= 0.8\linewidth]{Figures/A-schematic-representation-of-the-architecture-of-a-denoising-diffusion-probabilistic_2.jpg}
\caption{Forward and backward process in denoising diffusion models. These models initially map an input image to a noise image by gradually adding Gaussian noise in many small steps and subsequently learning to perform the reverse process in small steps as well \parencite{DDPM}. Thus, DDPMs are trained to predict what noise should be removed from a given image at a certain step in the denoising process. A popular implementation of DDPMs involves using a neural network, typically with Unet-shaped architecture, ResNet layers, time embeddings and attention layers. The U-Net is trained to predict the noise to be removed from an input image given the noisy input and given the step in the dffusin process chain \parencite{DDPM}. A trained DDPM can then generate synthetic images by iteratively removing noise from a pure Gaussian noisy input. Class-conditioning the DDPM allows one model to generate images with varying content, such as of a specific animal, or medical images belonging to a specific diagnosis. Image modified from \citeauthor{Kim2024} \parencite{Kim2024}.}

% OCT-A (OCTA-DONH, OCTA-SONH, OCTA-DMAC, OCTA-SMAC), structural OCT (OCT-BONH, OCT-BMAC) and fundus SLO (FAF) images }
\label{fig:fig:ddm_schema}
\end{figure}

==> Figures/correlations.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width=0.8 \textwidth]{Figures/correlations.jpg}
\caption{(A-D): Distributions for maximum pearson correlation values computed for $200$ synthetic images and all real images. Distributions display the highest correlation for image pairs among real images (RvR, orange), among synthetic images (SvS, green) and for all synthetic images with any real image (SVR, blue). Arrows compare the differences between SvR and RvR (black) and the differences between RvR and SvS (grey). WD values express the difference between two distributions with KS test p-values for the significance of such differences. pearsonr = Pearson's correlation coefficient. ** = p < 0.005}
\label{fig:correlations_synthetic_data}
\end{figure}


==> Introduction/Models.tex <==
The U-Net architecture typically consists of an encoder path and a decoder path. In this case, the encoder path starts with the input layer and gradually reduces the spatial dimensions through downsampling operations (such as max-pooling or convolutions). The decoder path then gradually upsamples the feature maps to the original input size

==> Methods/Cams.tex <==
\subsection{Class activation maps} With class activation maps (CAMs) we attempt at providing explanation to the black-box CNN predictions. CAMs indicate which discriminative image regions contribute to a model's output value. 
% We implemented Gradient-weighted CAM (Grad CAM) with the library \texttt{pytorch-grad-cam} to produce heatmaps that give insight into the model's activations after the last convolutional layer \parencite{Selvaraju2019}. Since the activity of convolutional layers often maps spatially to the input, we can upsample the GradCAM attributions to mask the input. GradCAM applied to our binary classification network computes the gradient of the binary output layer with respect to each of the network's activations at the selected convolutional layer. To produce the heatmap, the gradient at the output layer is computed and subsequently multiplied with the layer's activations. 
As our model outputs the probability for AmyloidPET- the resulting heatmap displays the image regions that, according to the model, contribute to an output of a higher probability of AmyloidPET-. 
% This is because our model has only 1 output layer for binary predictions, so the gradCAMs can only be calculated with respect to this one output node. If the output layer had been a 2-node layer we could have displayed heatmaps with respect to AmyloidPET+ predictions by calculating the gradient with respect to the corresponding output node. 




==> PAPER_GUIDELINES.tex <==
•	Title
•	Synopsis/Precis: a 35 word summary of the main findings or outcomes of the study for the 'At a Glance' article
•	Structured abstract: (250 words, headings: "Background/Aims", "Methods", "Results", and "Conclusion")
•	Introduction
•	Materials and methods
•	Results
•	Discussion

Clinical science: up to 3000 words, up to 5 images/tables,35 references 
Laboratory Science: up to 3000 words, up to 5 images/, 35 references 

Please include the key messages of your article after your abstract using the following headings. This section should be no more than 3-5 sentences and should be distinct from the abstract; be succinct, specific and accurate. 
•	What is already known on this topic - summarise the state of scientific knowledge on this subject before you did your study and why this study needed to be done
•	What this study adds - summarise what we now know as a result of this study that we did not know before
•	How this study might affect research, practice or policy - summarise the implications of this study
This will be published as a summary box after the abstract in the final published article.

https://authors.bmj.com/writing-and-formatting/
https://authors.bmj.com/writing-and-formatting/formatting-your-paper/ 
https://authors.bmj.com/before-you-submit/topic-collections/submitting-to-a-topic-collection/ 
https://www.icmje.org/recommendations/browse/manuscript-preparation/preparing-for-submission.html
https://www.bmj.com/about-bmj/resources-authors/article-submission/authorship-contributorship

https://www.bmj.com/sites/default/files/attachments/resources/2018/05/BMJ-InstructionsForAuthors-2018.pdf

==> Tables/classification_results_t.tex <==
\begin{table}[H]
\centering
\noindent\begin{tabular}{l|ll|ll|ll|ll}
\hline
                          & \multicolumn{2}{c|}{AUROC on validation} & \multicolumn{2}{c|}{AUPR on validation} & \multicolumn{2}{c|}{AUROC on test} & \multicolumn{2}{c}{AUPR on test}       \\
Classifier                & Baseline           & Pretrained          & Baseline           & Pretrained         & Baseline         & Pretrained      & Baseline             & Pretrained      \\ \hline
Unimodal                  & \textbf{}          &                     &                    & \textbf{}          &                  & \textbf{}       &                      & \textbf{}       \\
- OCTA-SMAC & 0.646              & 0.5826              & 0.7485             & 0.7149             & 0.381            & \textbf{0.5863} & 0.5315               & \textbf{0.675}  \\
- OCT-BONH              & 0.6016             & 0.7071              & 0.6832             & 0.7943             & 0.5303           & \textbf{0.5833} & 0.6466               & \textbf{0.6891} \\
- OCT-BMAC          & 0.6676             & 0.7279              & 0.7215             & 0.8031             & 0.3913           & \textbf{0.6152} & 0.5283               & \textbf{0.6828} \\
- FAF                      & 0.7419             & 0.6641              & 0.8681             & 0.7571             & \textbf{0.5491}  & 0.4777          & \textbf{0.7505}      & 0.6761          \\
Multimodal                &                    & \textbf{}           & \textbf{}          &                    & \textbf{}        &                 & \textbf{}            &                 \\
- without metadata        & 0.5667             & 0.7083              & 0.7517             & 0.7863             & \textbf{0.6071}  & 0.4911          & \textbf{0.7196}      & 0.6327          \\
- with metadata           & 0.6305             & 0.5917              & 0.7762             & 0.7786             & \textbf{0.7292}           & 0.369           & {\ul \textbf{0.848}} & 0.6256          \\ \hline
\end{tabular}
\caption{Classification results}
\label{tab:classification_results_old}
\end{table}


==> Tables/film_results.tex <==
\begin{table}[H]
\centering
\noindent\begin{tabular}{l|ll|ll|ll|ll}
\hline
                          & \multicolumn{2}{c|}{AUROC on validation} & \multicolumn{2}{c|}{AUPR on validation} & \multicolumn{2}{c|}{AUROC on test} & \multicolumn{2}{c}{AUPR on test}       \\
Classifier                & Baseline           & Pretrained          & Baseline           & Pretrained         & Baseline         & Pretrained      & Baseline             & Pretrained      \\ \hline
Mixed-modality            &                    &                     &                    &                    &                  &                 &                      &                 \\
- without FiLM            & 0.5853             & \textbf{}           & 0.6716             &          & 0.4492           &                 & \textbf{0.5952}               &                 \\
- with FiLM               & 0.5899             &                     & 0.6858             & \textbf{}          & 0.4157           & \textbf{}       & 0.5544               & \textbf{}    \\ \hline
\end{tabular}
\caption{AUROC and AUPR for classification by one mixed-modality classifier that predicts AmyloidPET status for all types of images. For comparison we implemented the mixed-modality classifier without FiLM layer and thus this model has no context on the modality of an input image. This network slightly underperforms on the test set compared to the classifier that is modality aware.}
\label{tab:film_results}
\end{table}


==> Tables/table_classification_t.tex <==
\begin{table}[]
\begin{tabular}{lllllllll}
\hline
Subset                          & \begin{tabular}[c]{@{}l@{}}{[}N{]} eyes \\ (All)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}\%{]} AmyloidPET+ \\ (All)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} eyes \\ (Train)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}\%{]} AmyloidPET+\\ (Train)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} eyes\\ (Val)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}\%{]} AmyloidPET+\\ (Val)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} eyes\\ (Test)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}\%{]} AmyloidPET+\\ (Test)\end{tabular} \\ \hline
\multicolumn{1}{l|}{Classification}   & 326                                                           &                                                                  &                                                                 &                                                                        &                                                              &                                                                      &                                                               &                                                                       \\
\multicolumn{1}{l|}{Unimodal}   & 285                                                           &                                                                       &                                                                 &                                                                        &                                                              &                                                                      &                                                               &                                                                       \\
\multicolumn{1}{l|}{\hspace{0.2cm}    OCTA-SMAC}  & 276                                                           & 0.388                                                                 & 168                                                             & 0.381                                                                  & 55                                                           & 0.4                                                                  & 53                                                            & 0.396                                                                 \\
\multicolumn{1}{l|}{\hspace{0.2cm}    OCT-BONH}   & 278                                                           & 0.378                                                                 & 164                                                             & 0.36                                                                   & 56                                                           & 0.429                                                                & 58                                                            & 0.379                                                                 \\
\multicolumn{1}{l|}{\hspace{0.2cm}    OCT-BMAC}   & 276                                                           & 0.388                                                                 & 166                                                             & 0.367                                                                  & 54                                                           & 0.426                                                                & 56                                                            & 0.411                                                                 \\
\multicolumn{1}{l|}{\hspace{0.2cm}    FAF}        & 250                                                           & 0.352                                                                 & 158                                                             & 0.348                                                                  & 48                                                           & 0.354                                                                & 44                                                            & 0.364                                                                 \\
\multicolumn{1}{l|}{Multimodal} & 198                                                           & 0.389                                                                 & 121                                                             & 0.397                                                                  & 39                                                           & 0.385                                                                & 38                                                            & 0.368                                                                 \\ \hline
\end{tabular}
\caption{Image data used for classification}
\label{tab:classification_data}
\end{table}

==> Tables/table_synthesis_t.tex <==
\begin{table}[]
\begin{tabular}{lllllllll}
\hline
Subset                         & \begin{tabular}[c]{@{}l@{}}{[}N{]} eyes \\ (All)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} Images \\ (All)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} eyes \\ (Dev)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} images \\ (Dev)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}\%{]} AmyloidPET+ \\ (Dev)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} eyes \\ (Test)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}N{]} images \\ (Test)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}\%{]} AmyloidPET+ \\ (Test)\end{tabular} \\ \hline
\multicolumn{1}{l|}{Synthesis} & 328                                &                                                                 &                                                               &                                                                 &                                                                       &                                                                &                                                                  &                                                                        \\
\multicolumn{1}{l|}{\hspace{0.2cm}OCTA-SMAC} & 276                                                           & 276                                                             & 223                                                           & 223                                                             & 0.386                                                                 & 53                                                             & 53                                                               & 0.396                                                                  \\
\multicolumn{1}{l|}{\hspace{0.2cm}OCT-BONH}  & 278                                                           & 278                                                             & 220                                                           & 220                                                             & 0.377                                                                 & 58                                                             & 58                                                               & 0.379                                                                  \\
\multicolumn{1}{l|}{\hspace{0.2cm}OCT-BMAC}  & 276                                                           & 276                                                             & 220                                                           & 220                                                             & 0.382                                                                 & 56                                                             & 56                                                               & 0.411                                                                  \\
\multicolumn{1}{l|}{\hspace{0.2cm}FAF}       & 254                                                           & 272                                                             & 210                                                           & 225                                                             & 0.351                                                                 & 44                                                             & 47                                                               & 0.34                                                                   \\ \hline
\end{tabular}
\caption{Data used for synthesis and training of filter}
\label{tab:synthesis_data}
\end{table}

==> Tables_old/table_classification.tex <==
\vspace{1em}
\begin{table}[H]
\begin{tabular}{@{}lllllll@{}}
\toprule
Subset                          & {[}N{]} eyes (All) & {[}\%{]} AmyloidPET+ (All) & {[}N{]} eyes (Train) & {[}\%{]} AmyloidPET+ (Train) & {[}N{]} eyes (Test) & {[}\%{]} AmyloidPET+ (Test) \\ \midrule
\multicolumn{1}{l|}{Included}   & 326                & 0.377                      & 262                  & 0.328                        & 64                  & 0.569                       \\
\multicolumn{1}{l|}{OCTA-DONH}  & 278                & 0.377                      & 220                  & 0.332                        & 58                  & 0.552                       \\
\multicolumn{1}{l|}{OCTA-SONH}  & 278                & 0.377                      & 220                  & 0.332                        & 58                  & 0.552                       \\
\multicolumn{1}{l|}{OCTA-DMAC}  & 276                & 0.384                      & 221                  & 0.33                         & 55                  & 0.6                         \\
\multicolumn{1}{l|}{OCTA-SMAC}  & 276                & 0.384                      & 221                  & 0.33                         & 55                  & 0.6                         \\
\multicolumn{1}{l|}{OCT-BONH}   & 278                & 0.377                      & 220                  & 0.332                        & 58                  & 0.552                       \\
\multicolumn{1}{l|}{OCT-BMAC}   & 276                & 0.384                      & 221                  & 0.33                         & 55                  & 0.6                         \\
\multicolumn{1}{l|}{FAF}        & 250                & 0.352                      & 199                  & 0.307                        & 51                  & 0.529                       \\
\multicolumn{1}{l|}{Multimodal} & 197                & 0.391                      & 154                  & 0.351                        & 43                  & 0.535                       \\ \bottomrule
\end{tabular}
\caption{Image data availability.}
\label{tab:ImageSubsets}
\end{table}

==> Tables_old/table_multimodal_results.tex <==

\begin{table}[htpb]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{2.1cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
\hline
& \multicolumn{2}{c|}{AUROC on validation}       & \multicolumn{2}{c|}{AUPR on validation}        & \multicolumn{2}{c|}{AUROC on test}             & \multicolumn{2}{c}{AUPR   on test}             \\
\hline
Modality   (fold) &  Baseline     & Pretrained         &  Baseline    & Pretrained         &  Baseline  & Pretrained      &  Baseline  & Pretrained       \\
\hline
Multimodal 1               & \textbf{0.890}       & \textbf{0.214}     & \textbf{0.931}       & \textbf{0.497}     & \textbf{0.504}       & 0.430              & \textbf{0.487}       & 0.412              \\
Multimodal 2               & \textbf{0.744}       & 0.772              & \textbf{0.897}       & \textbf{0.911}     & \textbf{0.541}       & \textbf{0.408}     & \textbf{0.494}       & \textbf{0.404}     \\
Multimodal 3               & \textbf{0.788}       & 0.571              & \textbf{0.858}       & \textbf{0.758}     & 0.470                & \textbf{0.520}     & 0.508                & \textbf{0.591}     \\
Multimodal 4               & \textbf{0.749}       & 0.647              & \textbf{0.846}       & 0.790              & \textbf{0.550}       & \textbf{0.459}     & \textbf{0.502}       & \textbf{0.461}     \\
Multimodal 5               & \textbf{0.309}       & 0.704              & \textbf{0.581}       & \textbf{0.838}     & \textbf{0.578}       & 0.478              & \textbf{0.590}       & 0.496              \\
\hline 
Average                    & \underline{\textbf{0.696}} & 0.582              & \underline{\textbf{0.823}} & 0.759              & \underline{\textbf{0.529}} & 0.459              & \underline{\textbf{0.516}} &  0.473     \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Multimodal classification}
\label{tab:multimodal_results}
\end{table}



==> Tables_old/table_splits.tex <==



\begin{table}[htbp]

\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|>{\raggedright\arraybackslash}p{2.1cm}|p{0.7cm}|p{0.7cm}|p{1.5cm}|p{1.5cm}|p{1.9cm}|p{0.7cm}|p{0.7cm}|p{1.5cm}|p{1.5cm}|p{1.9cm}|}
\hline
            & \multicolumn{5}{c|}{Train} & \multicolumn{5}{c|}{Validation} \\
\hline
Modality (fold)        & Images (N) & Eyes (N) & AmyloidPET+ Images (\%) & Multimodal eyes (N (\%)) & AmyloidPET+ Multimodal (\%) & Images (N) & Eyes (N) & AmyloidPET+ Images (\%) & Multimodal eyes (N (\%)) & AmyloidPET+ Multimodal (\%) \\
\hline
OCTA-DONH (1) & 177        & 174      & 0.337                   & 116 (0.667)              & 0.345                       & 46         & 46       & 0.298                   & 38 (0.826)               & 0.368                       \\
OCTA-DONH (2) & 177        & 175      & 0.313                   & 125 (0.714)              & 0.360                       & 46         & 45       & 0.396                   & 29 (0.644)               & 0.310                       \\
OCTA-DONH (3) & 181        & 178      & 0.324                   & 122 (0.685)              & 0.352                       & 42         & 42       & 0.344                   & 32 (0.762)               & 0.344                       \\
OCTA-DONH (4) & 174        & 173      & 0.338                   & 127 (0.734)              & 0.339                       & 49         & 47       & 0.286                   & 28 (0.596)               & 0.393                       \\
OCTA-DONH (5) & 183        & 180      & 0.329                   & 127 (0.706)              & 0.354                       & 40         & 40       & 0.325                   & 27 (0.675)               & 0.333                       \\
\hline
OCTA-SONH (1) & 177        & 174      & 0.337                   & 116 (0.667)              & 0.345                       & 46         & 46       & 0.298                   & 38 (0.826)               & 0.368                       \\
OCTA-SONH (2) & 181        & 178      & 0.313                   & 125 (0.702)              & 0.360                       & 42         & 42       & 0.396                   & 29 (0.690)               & 0.310                       \\
OCTA-SONH (3) & 181        & 178      & 0.324                   & 122 (0.685)              & 0.352                       & 42         & 42       & 0.344                   & 32 (0.762)               & 0.344                       \\
OCTA-SONH (4) & 171        & 168      & 0.338                   & 127 (0.756)              & 0.339                       & 52         & 52       & 0.286                   & 28 (0.538)               & 0.393                       \\
OCTA-SONH (5) & 182        & 182      & 0.329                   & 127 (0.698)              & 0.354                       & 41         & 38       & 0.325                   & 27 (0.711)               & 0.333                       \\
\hline
OCTA-DMAC (1) & 171        & 169      & 0.337                   & 116 (0.686)              & 0.345                       & 53         & 52       & 0.298                   & 38 (0.731)               & 0.368                       \\
OCTA-DMAC (2) & 186        & 183      & 0.313                   & 125 (0.683)              & 0.360                       & 38         & 38       & 0.396                   & 29 (0.763)               & 0.310                       \\
OCTA-DMAC (3) & 178        & 175      & 0.324                   & 122 (0.697)              & 0.352                       & 46         & 46       & 0.344                   & 32 (0.696)               & 0.344                       \\
OCTA-DMAC (4) & 177        & 176      & 0.338                   & 127 (0.722)              & 0.339                       & 47         & 45       & 0.286                   & 28 (0.622)               & 0.393                       \\
OCTA-DMAC (5) & 184        & 181      & 0.329                   & 127 (0.702)              & 0.354                       & 40         & 40       & 0.325                   & 27 (0.675)               & 0.333                       \\
\hline
OCTA-SMAC (1) & 177        & 174      & 0.337                   & 116 (0.667)              & 0.345                       & 47         & 47       & 0.298                   & 38 (0.809)               & 0.368                       \\
OCTA-SMAC (2) & 182        & 179      & 0.313                   & 125 (0.698)              & 0.360                       & 42         & 42       & 0.396                   & 29 (0.690)               & 0.310                       \\
OCTA-SMAC (3) & 177        & 174      & 0.324                   & 122 (0.701)              & 0.352                       & 47         & 47       & 0.344                   & 32 (0.681)               & 0.344                       \\
OCTA-SMAC (4) & 184        & 182      & 0.338                   & 127 (0.698)              & 0.339                       & 40         & 39       & 0.286                   & 28 (0.718)               & 0.393                       \\
OCTA-SMAC (5) & 176        & 175      & 0.329                   & 127 (0.726)              & 0.354                       & 48         & 46       & 0.325                   & 27 (0.587)               & 0.333                       \\
\hline
OCT-BONH (1)  & 169        & 166      & 0.337                   & 116 (0.699)              & 0.345                       & 54         & 54       & 0.298                   & 38 (0.704)               & 0.368                       \\
OCT-BONH (2)  & 182        & 179      & 0.313                   & 125 (0.698)              & 0.360                       & 41         & 41       & 0.396                   & 29 (0.707)               & 0.310                       \\
OCT-BONH (3)  & 183        & 180      & 0.324                   & 122 (0.678)              & 0.352                       & 40         & 40       & 0.344                   & 32 (0.800)               & 0.344                       \\
OCT-BONH (4)  & 180        & 179      & 0.338                   & 127 (0.709)              & 0.339                       & 43         & 41       & 0.286                   & 28 (0.683)               & 0.393                       \\
OCT-BONH (5)  & 178        & 176      & 0.329                   & 127 (0.722)              & 0.354                       & 45         & 44       & 0.325                   & 27 (0.614)               & 0.333                       \\
\hline
OCT-BMAC (1)  & 169        & 169      & 0.337                   & 116 (0.686)              & 0.345                       & 55         & 52       & 0.298                   & 38 (0.731)               & 0.368                       \\
OCT-BMAC (2)  & 185        & 182      & 0.313                   & 125 (0.687)              & 0.360                       & 39         & 39       & 0.396                   & 29 (0.744)               & 0.310                       \\
OCT-BMAC (3)  & 175        & 172      & 0.324                   & 122 (0.709)              & 0.352                       & 49         & 49       & 0.344                   & 32 (0.653)               & 0.344                       \\
OCT-BMAC (4)  & 183        & 180      & 0.338                   & 127 (0.706)              & 0.339                       & 41         & 41       & 0.286                   & 28 (0.683)               & 0.393                       \\
OCT-BMAC (5)  & 184        & 181      & 0.329                   & 127 (0.702)              & 0.354                       & 40         & 40       & 0.325                   & 27 (0.675)               & 0.333                       \\
\hline
FAF (1)       & 151        & 151      & 0.337                   & 116 (0.768)              & 0.345                       & 48         & 48       & 0.298                   & 38 (0.792)               & 0.368                       \\
FAF (2)       & 164        & 164      & 0.313                   & 125 (0.762)              & 0.360                       & 35         & 35       & 0.396                   & 29 (0.829)               & 0.310                       \\
FAF (3)       & 160        & 160      & 0.324                   & 122 (0.762)              & 0.352                       & 39         & 39       & 0.344                   & 32 (0.821)               & 0.344                       \\
FAF (4)       & 160        & 160      & 0.338                   & 127 (0.794)              & 0.339                       & 39         & 39       & 0.286                   & 28 (0.718)               & 0.393                       \\
FAF (5)       & 161        & 161      & 0.329                   & 127 (0.789)              & 0.354                       & 38         & 38       & 0.325                   & 27 (0.711)               & 0.333     \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Your caption here}
\label{tab:fold_descriptions}
\end{table}



==> Tables_old/table_unimodal_results.tex <==
\begin{table}[htbp]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{3cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
\hline
                                     & \multicolumn{3}{c|}{Validation} & \multicolumn{3}{c}{Test set} \\ 
\hline
Modality (fold) & AUROC      & AUPR       & AUPRG     & AUROC    & AUPR     & AUPRG   \\
\hline
FAF (1)         & 0.729      & 0.858      & 0.269     & 0.694    & 0.606    & 0.458   \\
FAF (2)         & 0.607      & 0.708      & 0.239     & 0.441    & 0.417    & 0.056   \\
FAF (3)         & 0.757      & 0.826      & 0.446     & 0.509    & 0.504    & 0.041   \\
FAF (4)         & 0.633      & 0.762      & 0.260     & 0.454    & 0.471    & 0.002   \\
FAF (5)         & 0.663      & 0.823      & 0.283     & 0.644    & 0.553    & 0.374   \\
\hline
OCT-BMAC (1)    & 0.510      & 0.744      & 0.001     & 0.640    & 0.567    & 0.362   \\
OCT-BMAC (2)    & 0.700      & 0.846      & 0.160     & 0.635    & 0.544    & 0.307   \\
OCT-BMAC (3)    & 0.614      & 0.715      & 0.226     & 0.551    & 0.503    & 0.216   \\
OCT-BMAC (4)    & 0.624      & 0.726      & 0.293     & 0.566    & 0.487    & 0.194   \\
OCT-BMAC (5)    & 0.410      & 0.627      & 0.000     & 0.517    & 0.504    & 0.078   \\
\hline
OCT-BONH (1)    & 0.702      & 0.869      & 0.314     & 0.525    & 0.468    & 0.048   \\
OCT-BONH (2)    & 0.292      & 0.542      & 0.000     & 0.433    & 0.417    & 0.003   \\
OCT-BONH (3)    & 0.646      & 0.747      & 0.265     & 0.448    & 0.439    & 0.002   \\
OCT-BONH (4)    & 0.613      & 0.803      & 0.131     & 0.501    & 0.546    & 0.004   \\
OCT-BONH (5)    & 0.662      & 0.745      & 0.273     & 0.519    & 0.520    & 0.065   \\
\hline
OCTA-DMAC (1)   & 0.645      & 0.817      & 0.265     & 0.540    & 0.473    & 0.098   \\
OCTA-DMAC (2)   & 0.474      & 0.658      & 0.135     & 0.579    & 0.565    & 0.238   \\
OCTA-DMAC (3)   & 0.584      & 0.791      & 0.018     & 0.511    & 0.452    & 0.063   \\
OCTA-DMAC (4)   & 0.729      & 0.836      & 0.451     & 0.490    & 0.439    & 0.138   \\
OCTA-DMAC (5)   & 0.669      & 0.762      & 0.262     & 0.530    & 0.510    & 0.119   \\
\hline
OCTA-DONH (1)   & 0.669      & 0.829      & 0.210     & 0.444    & 0.461    & 0.004   \\
OCTA-DONH (2)   & 0.654      & 0.672      & 0.359     & 0.560    & 0.517    & 0.166   \\
OCTA-DONH (3)   & 0.493      & 0.707      & 0.094     & 0.314    & 0.359    & 0.000   \\
OCTA-DONH (4)   & 0.726      & 0.858      & 0.280     & 0.582    & 0.542    & 0.148   \\
OCTA-DONH (5)   & 0.542      & 0.756      & 0.000     & 0.538    & 0.514    & 0.032   \\
\hline
OCTA-SMAC (1)   & 0.458      & 0.683      & 0.000     & 0.324    & 0.324    & 0.000   \\
OCTA-SMAC (2)   & 0.664      & 0.733      & 0.383     & 0.690    & 0.611    & 0.429   \\
OCTA-SMAC (3)   & 0.462      & 0.688      & 0.024     & 0.433    & 0.360    & 0.013   \\
OCTA-SMAC (4)   & 0.671      & 0.796      & 0.250     & 0.511    & 0.431    & 0.036   \\
OCTA-SMAC (5)   & 0.699      & 0.844      & 0.350     & 0.536    & 0.442    & 0.128   \\
\hline
OCTA-SONH (1)   & 0.563      & 0.772      & 0.002     & 0.512    & 0.454    & 0.034   \\
OCTA-SONH (2)   & 0.633      & 0.717      & 0.199     & 0.642    & 0.610    & 0.328   \\
OCTA-SONH (3)   & 0.658      & 0.827      & 0.157     & 0.553    & 0.554    & 0.100   \\
OCTA-SONH (4)   & 0.640      & 0.824      & 0.210     & 0.401    & 0.418    & 0.000   \\
OCTA-SONH (5)   & 0.610      & 0.830      & 0.021     & 0.433    & 0.430    & 0.007   \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Your caption here}
\label{tab:unimodal_results}
\end{table}



==> Tables_old/table_unimodal_results_with_finetuned.tex <==

\begin{table}[htpb]
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{2.1cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
\hline
& \multicolumn{2}{c|}{AUROC on validation}       & \multicolumn{2}{c|}{AUPR on validation}        & \multicolumn{2}{c|}{AUROC on test}             & \multicolumn{2}{c}{AUPR   on test}             \\
\hline
Modality   (fold) &  Baseline     & Pretrained         &  Baseline    & Pretrained         &  Baseline  & Pretrained      &  Baseline  & Pretrained       \\
FAF (1)           & 0.729               & \textbf{0.773}    & 0.858              & \textbf{0.911}    & \textbf{0.694}   & 0.566          & \textbf{0.606}   & 0.521           \\
FAF (2)           & \textbf{0.607}      & 0.583             & 0.708              & \textbf{0.763}    & 0.441            & \textbf{0.460} & 0.417            & \textbf{0.455}  \\
FAF (3)           & \textbf{0.757}      & 0.746             & 0.826              & \textbf{0.859}    & 0.509            & \textbf{0.546} & 0.504            & \textbf{0.615}  \\
FAF (4)           & \textbf{0.633}      & 0.435             & \textbf{0.762}     & 0.719             & 0.454            & \textbf{0.713} & 0.471            & \textbf{0.702}  \\
FAF (5)           & \textbf{0.663}      & 0.623             & \textbf{0.823}     & 0.774             & \textbf{0.644}   & 0.347          & \textbf{0.553}   & 0.428           \\
\hline
Average           &\underline{\textbf{0.678}}          & 0.632  & 0.732              &  \underline{\textbf{0.735}}    &  \underline{\textbf{0.582}}   & \textbf{0.517} &  \underline{\textbf{0.521}}   & \textbf{0.463}  \\
\hline
OCT-BMAC (1)      & 0.510               & \textbf{0.561}    & 0.744              & \textbf{0.787}    & \textbf{0.640}   & 0.547          & 0.567            & \textbf{0.572}  \\
OCT-BMAC (2)      & 0.700               & \textbf{0.722}    & \textbf{0.846}     & 0.772             & \textbf{0.635}   & 0.521          & \textbf{0.544}   & 0.414           \\
OCT-BMAC (3)      & \textbf{0.614}      & 0.579             & \textbf{0.715}     & 0.668             & \textbf{0.551}   & 0.456          & \textbf{0.503}   & 0.384           \\
OCT-BMAC (4)      & \textbf{0.624}      & 0.500             & \textbf{0.726}     & 0.695             & \textbf{0.566}   & 0.517          & \textbf{0.487}   & 0.425           \\
OCT-BMAC (5)      & 0.410               & \textbf{0.593}    & 0.627              & \textbf{0.751}    & 0.517            & \textbf{0.544} & 0.504            & \textbf{0.521}  \\
\hline
Average           & 0.572               & \underline{\textbf{0.591}}    & 0.732              & \textbf{0.735}    & \underline{\textbf{0.582}}   & \underline{\textbf{0.517}} & \underline{\textbf{0.521}}   & \underline{\textbf{0.463}}  \\
\hline
OCT-BONH (1)      & \textbf{0.702}      & 0.566             & \textbf{0.869}     & 0.796             & \textbf{0.525}   & 0.470          & 0.468            & \textbf{0.548}  \\
OCT-BONH (2)      & 0.292               & \textbf{0.559}    & 0.542              & \textbf{0.650}    & 0.433            & \textbf{0.579} & 0.417            & \textbf{0.524}  \\
OCT-BONH (3)      & \textbf{0.646}      & 0.558             & \textbf{0.747}     & 0.720             & 0.448            & \textbf{0.511} & 0.439            & \textbf{0.474}  \\
OCT-BONH (4)      & \textbf{0.613}      & 0.492             & \textbf{0.803}     & 0.718             & 0.501            & \textbf{0.571} & 0.546            & \textbf{0.571}  \\
OCT-BONH (5)      & 0.662               & 0.662             & 0.745              & \textbf{0.809}    & \textbf{0.519}   & 0.501          & \textbf{0.520}   & 0.485           \\
\hline
Average           & \underline{\textbf{0.583}}      & 0.567             & \underline{\textbf{0.741}}     & 0.739             & 0.485            & \underline{\textbf{0.526}} & 0.478            & \underline{\textbf{0.520}}   \\
\hline
OCTA-DMAC (1)     & \textbf{0.645}      & 0.422             & \textbf{0.817}     & 0.662             & \textbf{0.540}   & 0.534          & 0.473            & \textbf{0.530}  \\
OCTA-DMAC (2)     & 0.474               & \textbf{0.625}    & \textbf{0.658}     & 0.739             & 0.579            & \textbf{0.592} & \textbf{0.565}   & 0.540           \\
OCTA-DMAC (3)     & \textbf{0.584}      & 0.511             & \textbf{0.791}     & 0.647             & 0.511            & \textbf{0.517} & 0.452            & 0.429           \\
OCTA-DMAC (4)     & \textbf{0.729}      & 0.344             & \textbf{0.836}     & 0.655             & 0.490            & \textbf{0.579} & 0.439            & \textbf{0.533}  \\
OCTA-DMAC (5)     & \textbf{0.669}      & 0.379             & \textbf{0.762}     & 0.590             & \textbf{0.530}   & 0.369          & \textbf{0.510}   & 0.398           \\
\hline
Average           & \underline{\textbf{0.620}}       & 0.456             & \underline{\textbf{0.773}}     & 0.659             & \underline{\textbf{0.530}}    & 0.518          & \underline{\textbf{0.488}}   & 0.486           \\

\hline
OCTA-DONH (1)     & \textbf{0.669}      & 0.625             & \textbf{0.829}     & 0.774             & \textbf{0.444}   & 0.327          & \textbf{0.461}   & 0.385           \\
OCTA-DONH (2)     & \textbf{0.654}      & 0.577             & 0.672              & \textbf{0.646}    & \textbf{0.560}   & 0.534          & \textbf{0.517}   & 0.513           \\
OCTA-DONH (3)     & 0.493               & \textbf{0.610}    & 0.707              & \textbf{0.743}    & \textbf{0.314}   & 0.297          & 0.359            & \textbf{0.418}  \\
OCTA-DONH (4)     & \textbf{0.726}      & 0.673             & \textbf{0.858}     & 0.838             & \textbf{0.582}   & 0.394          & \textbf{0.542}   & 0.396           \\
OCTA-DONH (5)     & 0.542               & \textbf{0.637}    & 0.756              & \textbf{0.815}    & \textbf{0.538}   & 0.618          & 0.514            & \textbf{0.562}  \\
\hline
Average           & \underline{\textbf{0.617}}      & \underline{\textbf{0.624}}    & \underline{\textbf{0.764}  }   & 0.763             &\underline{\textbf{0.487}}   & 0.434          & \underline{\textbf{0.479}}   & 0.455           \\

\hline
OCTA-SMAC (1)     & 0.458               & 0.452             & \textbf{0.683}     & 0.636             & 0.324            & \textbf{0.494} & 0.324            & \textbf{0.415}  \\
OCTA-SMAC (2)     & \textbf{0.664}      & 0.500             & \textbf{0.733}     & 0.560             & \textbf{0.690}   & 0.530          & \textbf{0.611}   & 0.407           \\
OCTA-SMAC (3)     & \textbf{0.462}      & 0.431             & \textbf{0.688}     & 0.648             & 0.433            & \textbf{0.618} & 0.360            & \textbf{0.603}  \\
OCTA-SMAC (4)     & \textbf{0.671}      & 0.451             & \textbf{0.796}     & 0.702             & 0.511            & \textbf{0.507} & 0.431            & \textbf{0.437}  \\
OCTA-SMAC (5)     & \textbf{0.699}      & 0.541             & \textbf{0.844}     & 0.732             & \textbf{0.536}   & 0.492          & \textbf{0.442}   & 0.440           \\
\hline
Average           & \underline{\textbf{0.591}}      & 0.475             & \underline{\textbf{0.749}}     & 0.656             & 0.499            & \underline{\textbf{0.528}} & 0.434            &\underline{\textbf{0.461}}  \\

\hline
OCTA-SONH (1)     & 0.563               & \textbf{0.594}    & \textbf{0.772}     & 0.729             & \textbf{0.512}   & 0.431          & \textbf{0.454}   & 0.448           \\
OCTA-SONH (2)     & \textbf{0.633}      & 0.459             & \textbf{0.717}     & 0.585             & 0.642            & \textbf{0.653} & \textbf{0.610}   & 0.598           \\
OCTA-SONH (3)     & \textbf{0.658}      & 0.571             & \textbf{0.827}     & 0.676             & \textbf{0.553}   & 0.483          & \textbf{0.554}   & 0.425           \\
OCTA-SONH (4)     & \textbf{0.640}      & 0.607             & \textbf{0.824}     & 0.746             & 0.401            & \textbf{0.480} & 0.418            & \textbf{0.474}  \\
OCTA-SONH (5)     & \textbf{0.610}      & 0.453             & \textbf{0.830}     & 0.684             & 0.433            & \textbf{0.584} & 0.430            & \textbf{0.477} 
\\
\hline
Average           & \underline{\textbf{0.621}}      & 0.537             & \underline{\textbf{0.794}}     & 0.684             & 0.508            & \underline{\textbf{0.526}} &\underline{\textbf{0.493}}   & 0.484          \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Unimodal classification}
\label{tab:unimodal_results_with_finetune}
\end{table}


